Unsupervised Cross-lingual Representation Learning for Speech Recognition

This paper presents XLSR which learns cross-lingual speech representations by pretraining a single model from the raw waveform of speech in multiple languages. We build on wav2vec 2.0 which is trained by solving a contrastive task over masked latent speech representations and jointly learns a quantization of the latents shared across languages. The resulting model is fine-tuned on labeled data and experiments show that cross-lingual pretraining significantly outperforms monolingual pretraining. On the CommonVoice benchmark, XLSR shows a relative phoneme error rate reduction of 72% compared to the best known results. On BABEL, our approach improves word error rate by 16% relative compared to a comparable system. Our approach enables a single multilingual speech recognition model which is competitive to strong individual models. Analysis shows that the latent discrete speech representations are shared across languages with increased sharing for related languages. We hope to catalyze research in low-resource speech understanding by releasing XLSR-53, a large model pretrained in 53 languages.

==> XLSR [ICLR 2021] (1)/macro.tex <==
%!TEX root = main.tex

\renewcommand{\Re}{\mathbb{R}}

\newcommand*\samethanks[1][\value{footnote}]{\footnotemark[#1]}
\newcommand*\residency[1][\value{footnote}]{\footnotemark[#1]}

\newcommand{\ma}[1]{\textcolor{orange}{#1}}
\newcommand{\alexei}[1]{\textcolor{purple}{#1}}
\newcommand{\alexis}[1]{\textcolor{blue}{#1}}
\newcommand{\comment}[1]{\textcolor{red}{TODO: \emph{#1}}}
\newcommand{\replace}[2]{\textcolor{red}{\st{#1}}{\textcolor{blue}{ {#2} }}}

\newcommand{\wvpp}{wav2vec 2.0}
\newcommand{\xlsr}{XLSR}
\newcommand{\wvppbase}{\wvpp{} Base}
\newcommand{\wvppbig}{\wvpp{} Large}

\newcommand{\Inp}{\mathcal{X}}
\newcommand{\Feat}{\mathcal{Z}}
\newcommand{\QFeat}{\mathcal{Q}}
\newcommand{\Context}{\mathcal{C}}
% \newcommand{\R}{\mathbb{R}}

\newcommand{\ze}{\mathbf{z}}
\newcommand{\zq}{\mathbf{q}}
\newcommand{\zqt}{\mathbf{\tilde{q}}}
\newcommand{\cc}{\mathbf{c}}
\newcommand{\e}{\mathbf{e}}

\renewcommand{\sectionautorefname}{\textsection} 
\renewcommand{\subsectionautorefname}{\textsection} 
\renewcommand{\subsubsectionautorefname}{\textsection} 

==> XLSR [ICLR 2021] (1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> XLSR [ICLR 2021] (1)/tables.tex <==


% Results of BABEL on "in-pretraining" languages
\newcommand{\insertBABELtableone}{
    \begin{table*}[t]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l|cc| cccccccccc|c}
            \toprule
            {\bf Model} & {\bf \#pt} & {\bf \#ft} & {\bf bn} & {\bf zh} & {\bf ka} & {\bf ht} & {\bf ku} & {\bf ps} & {\bf ta} & {\bf tr} & {\bf tp} & {\bf vi} & {\bf Avg}\\
                \midrule
                \midrule
                \multicolumn{3}{l|}{Number of pretraining hours per language} & 56h & 130h & 46h & 61h & 38h & 71h & 63h & 70h & 36h & \multicolumn{1}{c|}{79h} & 650h  \\
                \multicolumn{3}{l|}{Number of fine-tuning hours per language} & 56h & 130h & 46h & 61h & 38h & 71h & 63h & 70h & 36h & \multicolumn{1}{c|}{79h} & 650h  \\
                \midrule
                \midrule
                \multicolumn{14}{l}{\it Baselines from previous work} \\
                \midrule
                Mono-BLSTMP~\citep{cho2018multiseq2seq} &  10 & 1 & 43.4 & 37.4 & 35.4 & 39.7 & 55.0 & 37.3 & 55.3 & 50.3 & 32.7 & 54.3 & 44.1 \\
                Multi-BLSTMP~\citep{cho2018multiseq2seq} &  10 & 1 & 42.9 & 36.3 & 38.9 & 38.5 & 52.1 & 39.0 & 48.5 & 36.4 & 31.7 & 41.0 & 40.5 \\
                + VGG~\citep{cho2018multiseq2seq} &  10 & 1 & 39.6 & 34.3 & 36.0 & 34.5 & 49.9 & 34.7 & 45.5 & 28.7 & 33.7 & 37.4 & 37.4 \\
                \midrule
                \multicolumn{14}{l}{\it Our monolingual models} \\
                \midrule
                Training from scratch &  1 & 1 & 47.6 & 42.7 & 45.0 & 45.0 & 58.4 & 43.2 & 55.7 & 44.6 & 45.2 & 43.6 & 47.1 \\
                % XLSR-En &  1 & 1 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0   \\
                XLSR-Monolingual &  1 & 1 & 31.8 & 28.0 & 30.5 & 27.9 & 46.9 & 25.5 & 36.0 & 26.1 & 26.8 & 25.2 & 30.5 \\
                \midrule
                \multicolumn{14}{l}{\it Our multilingual models} \\
                \midrule
                XLSR-10 &  10 & 1 & 26.6 & 24.7 & 21.8 & 23.2 & 38.2 & 22.6 & 30.5 & 22.3 & 17.3 & 21.7 & 24.9 \\
                XLSR-10 (separate vocab) &  10 & 10 & 29.5 & 29.1 & 25.9 & 26.5 & 40.4 & 25.8 & 33.4 & 24.6 & 19.3 & 24.3 & 27.9  \\
                \midrule
                \multicolumn{14}{l}{\it Our multilingual models (Large)} \\
                \midrule
                XLSR-10 &  10 & 1 & 25.1 & \bf 23.4 & 19.7 & 21.1 & 36.8 & 21.6 & 28.6 & 19.8 & 16.1 & \bf 19.9 & 23.2 \\
                XLSR-10 (separate vocab) &  10 & 10 & 25.8 & 25.0 & 20.7 & 22.0 & 37.2 & 21.2 & 28.9 & 19.9 & 15.9 & 20.7 & 23.7 \\
                \midrule
                \multicolumn{14}{l}{\it Our Large XLSR-53 model pretrained on 56k hours} \\
                \midrule
                XLSR-53 & 53 & 1 & \bf 24.3 & 25.4 & \bf 17.2 & \bf 19.0 & \bf 35.4 & \bf 20.7 & \bf 27.4 & \bf 18.8 & \bf 13.7 & 21.8 & \bf 22.4 \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{BABEL results using character error rate (CER) on in-pretraining languages.} Baseline results are from~\citet{cho2018multiseq2seq} and use the same amount of data as our multilingual models. 
            %We pretrain our models on either one language ($\text{pt} = 1$) or $N=10$ languages ($\text{pt} = N$); and fine-tune our model on each language ($\text{ft} = 1$) or all languages ($\text{ft} = N$).
            \label{tab:bbl_results1}}
        \end{center}
       \vspace{-0.3cm}
    \end{table*}
}

% Results of BABEL on "out-of-pretraining" languages + trade-off analysis
\newcommand{\insertBABELtabletwo}{
\begin{table*}[t]
	\begin{minipage}[b]{0.48\linewidth}
        \begin{center}
            % \scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{l|cc|cccc|c}
            \toprule
            % \multicolumn{3}{c}{\#hours for pretraining} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {\bf Model} & {\bf \#pt} & {\bf \#ft} & {\bf as} & {\bf tl} & {\bf sw} & {\bf lo} & {\bf Avg} \\
                \midrule
                \midrule
                \multicolumn{3}{l|}{Number of pretraining hours} & 55h & 76h & 30h & \multicolumn{1}{c|}{59h} & 220h  \\
                \multicolumn{3}{l|}{Number of fine-tuning hours} & 55h & 76h & 30h & \multicolumn{1}{c|}{59h} & 220h  \\
                \midrule
                \midrule
                \multicolumn{8}{l}{\it Baselines from previous work} \\
                \midrule
                Monolingual~\citep{cho2018multiseq2seq} &  10 & 1 & 45.6 & 43.1 & 33.1 & 42.1 & 41.0 \\
                Stage-2 retraining~\citep{cho2018multiseq2seq} &  10 & 1 & 41.3 & 37.9 & 29.1 & 38.7 & 36.8 \\
                \midrule
                \multicolumn{8}{l}{\it Our monolingual models} \\
                \midrule
                Training from scratch & 1 & 1 & 50.2 & 41.7 & 40.8 & 43.5 & 44.1 \\
                XLSR-Monolingual &  1 & 1 & 34.8 & 25.4 & 26.8 & 29.1 & 29.0 \\
                \midrule
                \multicolumn{8}{l}{\it Our multilingual models} \\
                \midrule
                XLSR-10 &  10 & 1 & 29.4 & 21.9 & 16.6 & 23.3 & 22.8 \\
                XLSR-10 (Large) & 10 & 1 & 27.7 & 19.6 & 14.9 & 21.8 & 21.0 \\
                \midrule
                XLSR-53 (Large) & 53 & 1 & \bf 17.9 & \bf 13.1 & \bf 21.3 & \bf 22.4 & \bf 18.7 \\
                % \midrule
            % \multicolumn{3}{c}{\#hours (pretraining)} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\

                \bottomrule
            \end{tabular}
            }
            \captionof{table}{\textbf{BABEL results on out-of-pretraining languages (CER)}\label{tab:bbl_results2}. XLSR-10 provides strong representations for languages not seen during pretraining, outperforming monolingual models pretrained specifically on these languages.}
        \end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[b]{0.48\linewidth}
        \begin{center}
            % \scriptsize
            \resizebox{\linewidth}{!}{
            \begin{tabular}[t]{l |cc| ccccc}
            \toprule
            % \multicolumn{3}{c}{\#hours for pretraining} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\
            % \midrule
            {\bf Model} & {\bf \#pt} & {\bf \#ft} & {\bf as} & {\bf tl} & {\bf sw} & {\bf lo} & {\bf ka}\\
                \midrule
                \midrule
                \multicolumn{3}{l|}{Number of pretraining hours} & 55h & 76h & 30h & 59h  & 46h \\
                \multicolumn{3}{l|}{Number of fine-tuning hours} & 55h & 76h & 30h & 59h & 46h \\
                \midrule
                \midrule
                \multicolumn{8}{l}{\it Baselines from previous work} \\
                \midrule
                \cite{alumae2016georgian} & 1 & 1 & - & - & - & - & 32.2 \\
                \cite{ragni2018confidence} & 1 & 1 & - & 40.6 &  35.5 & - & - \\
                % Multi-10~\citep{inaguma2019transfer} &  10 & 1 & 53.6 & 46.2 & 41.6 & 45.9 & - \\
                \cite{inaguma2019transfer} &  1 & 1 & 49.1 & 46.3 & 38.3 & 45.7 & - \\
                \midrule
                \multicolumn{8}{l}{\it Our approach (no LM)} \\
                \midrule
                XLSR-10 (Large) &  10 & 1 & 49.1 & 40.6 & 38.1 & 34.7 & - \\
                \midrule
                \multicolumn{8}{l}{\it Our approach (4-gram KenLM)} \\
                \midrule
                XLSR-10 (Large) &  10 & 1 & 44.9 & 37.3 &  35.5 &  32.2 & - \\
                \midrule
                XLSR-53 (Large) & 53 & 1 & \bf 44.1 & \bf 33.2 & \bf 26.5 & \bf - &  \bf 31.1\\

                % \midrule
            % \multicolumn{3}{c}{\#hours (pretraining)} & 75h & 13h & 45h & \multicolumn{1}{l}{10h} & \\

                \bottomrule
            \end{tabular}
            }
            \captionof{table}{\textbf{BABEL results on out-of-pretraining languages using word error rate (WER).} We report baselines from previous work, including the strong \cite{alumae2016georgian} baseline. We report WER with and without 4-gram KenLM.
            \label{tab:bbl_sota}}
        \end{center}
    \end{minipage}
%       \vspace{-0.4cm}
    \end{table*}
}


% Results of CommonVoice on "in-pretraining" languages
\newcommand{\insertCVtable}{
    \begin{table*}[t]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l|ccc|cccccccccc|c}
            \toprule
            {\bf Model} & {\bf D} & {\bf \#pt} & {\bf \#ft} & {\bf es} & {\bf fr} & {\bf it} & {\bf ky} & {\bf nl} & {\bf ru} & {\bf sv} & {\bf tr} & {\bf tt} & {\bf zh} & {\bf Avg}\\
                \midrule
                \midrule
                \multicolumn{4}{l|}{Number of pretraining hours per language} & 168h & 353h & 90h & 17h & 29h & 55h & 3h & 11h & 17h &  \multicolumn{1}{c|}{50h} & 793h  \\
                \multicolumn{4}{l|}{Number of fine-tuning hours per language} & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h &  \multicolumn{1}{c|}{1h} & 10h  \\
                \midrule
                \midrule
                \multicolumn{15}{l}{\it Baselines from previous work} \\
                \midrule
                m-CPC$^{\dagger}$~\citep{rivire2020unsupervised} & LS$_{\text{100h}}$  & 10 & 1 & 38.7 & 49.3 & 42.1 & 40.7 & 44.4 & 45.2 & 48.8 & 49.7 & 44.0 & 55.5 & 45.8 \\
                m-CPC$^{\dagger}$~\citep{rivire2020unsupervised} & LS$_{\text{360h}}$  & 10 & 1 & 38.0 & 47.1 & 40.5 & 41.2 & 42.5 & 43.7 & 47.5 & 47.3 & 42.0 & 55.0 & 44.5 \\
                Fer et al.$^{\dagger}$~\citep{fer2017multilingually} & BBL$_{\text{all}}$  & 10 & 1 & 36.6 & 48.3 & 39.0 & 38.7 & 47.9 & 45.2 & 52.6 & 43.4 & 42.5 & 54.3 & 44.9 \\
                \midrule
                \multicolumn{15}{l}{\it Our monolingual models} \\
                \midrule
                XLSR-English & CV$_{\text{en}}$  & 1 & 1 & 13.7 & 20.0 & 19.1 & 13.2 & 19.4 & 18.6 & 21.1 & 15.5 & 11.5 & 27.1 & 17.9 \\
                % XLSR-En & LS-10k & all & eac & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00 & 00  \\
                XLSR-Monolingual & \ CV$_{\text{mo}}$  & 1 & 1 & 6.8 & 10.4 & 10.9 & 29.6 & 37.4 & 11.6 & 63.6 & 44.0 & 21.4 & 31.4 & 26.7 \\
                \midrule
                \multicolumn{15}{l}{\it Our multilingual models} \\
                \midrule
                XLSR-10 (unbalanced) & CV$_{\text{all}}$  & 10 & 1 & 9.7 & 13.6 & 15.2 & 11.1 & 18.1 & 13.7 & 21.4 & 14.2 & 9.7 & 25.8 & 15.3 \\
                XLSR-10 & CV$_{\text{all}}$  & 10 & 1 & 9.4 & 14.2 & 14.1 & 8.4 & 16.1 & 11.0 & 20.7 & 11.2 & 7.6 & 24.0 & 13.6 \\
                XLSR-10 (separate vocab) & CV$_{\text{all}}$  & 10 & 10 & 10.0 & 13.8 & 14.0 & 8.8 & 16.5 & 11.6 & 21.4 & 12.0 & 8.7 & 24.5 & 14.1 \\
                XLSR-10 (shared vocab) & CV$_{\text{all}}$  & 10 & 10 & 9.4 & 13.4 & 13.8 & 8.6 & 16.3 & 11.2 & 21.0 & 11.7 & 8.3 & 24.5 & 13.8 \\
                \midrule
                \multicolumn{15}{l}{\it Our multilingual models (Large)} \\
                \midrule
                XLSR-10 & CV$_{\text{all}}$  & 10 & 1 & 7.9 & 12.6 & 11.7 & 7.0 & 14.0 & 9.3 & 20.6 & 9.7 & 7.2 & 22.8 & 12.3 \\
                XLSR-10 (separate vocab) & CV$_{\text{all}}$  & 10 & 10 & 8.1 & 12.1 & 11.9 & 7.1 & 13.9 & 9.8 & 21.0 & 10.4 & 7.6 & 22.3 & 12.4 \\
                XLSR-10 (shared vocab) & CV$_{\text{all}}$  & 10 & 10 & 7.7 & 12.2 & 11.6 & 7.0 & 13.8 & 9.3 & 20.8 & 10.1 & 7.3 & 22.3 & 12.2 \\
                \midrule
                \multicolumn{14}{l}{\it Our Large XLSR-53 model pretrained on 56k hours} \\
                \midrule
                XLSR-53 & D$_{\text{53}}$ & 53 & 1 & \bf 2.9 & \bf 5.0 & \bf 5.7 & \bf 6.1 & \bf 5.8 & \bf 8.1 & \bf 12.2 & \bf 7.1 & \bf 5.1 & \bf 18.3 & \bf 7.6 \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{CommonVoice phoneme error rate (PER).} Models are pretrained on either one language ($\text{pt} = 1$) or 10 languages ($\text{pt} = 10$); and fine-tuned on each language ($\text{ft} = 1$) or all languages ($\text{ft} = 10$). D indicates the pretraining data, LS for English LibriSpeech (100h or 360h), BBL$_{\text{all}}$ for BABEL (1070h), CV$_{\text{En}}$ for English CommonVoice (1350h), CV$_{\text{mo}}$ for monolingual (see number of pretraining hours per language) and CV$_{\text{all}}$ for multilingual (1350h). Languages can be high-resource (es, fr, it) or low-resource (e.g. ky, sv, tr, tt). Baseline results $^{\dagger}$ are from~\citet{rivire2020unsupervised}.
            %Multilingual pretraining shows strong improvements over monolingual models for low-resource languages (e.g. ky, sv, tr, tt), but are outperformed on high-resource languages (es, fr, it) - known as the transfer-interference trade-off~\citep{arivazhagan2019massively,conneau2019xlmr}. 
            %Upsampling low-resource languages (XLSR-10)~\citep{devlin2018bert,lample2019xlm} leads to better performance overall than the unbalanced setting (unb). 
            %Finally, we show the that a single model for all languages is possible via  multilingual fine-tuning: our Large XLSR-10 (shared vocab) obtains the best average performance of 12.2 PER.
            \label{tab:cv_results}}
        \end{center}
       \vspace{-0.3cm}
    \end{table*}
}


% Low-resource language and language similarity
\newcommand{\insertlangsim}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{0.8\linewidth}{!}{
            \begin{tabular}[h!]{l|cc|c|ccccccc}
            \toprule
                Model & {\bf \#pt} & {\bf \#ft} & {\bf it }& {\bf it }& {\bf es }& {\bf de }& {\bf en }& {\bf ru }& {\bf ka} & {\bf zh} \\
                \midrule
                \midrule
                \multicolumn{3}{l|}{Number of pretraining hours} & 5h (it) & \multicolumn{7}{c}{5h (it) + 50h (<lang>)} \\
                \midrule
                \midrule
                XLSR-Monolingual &  1 & 1 & 47.6 & 16.8 & 24.3 & 25.4 & 27 & 27.2 & 28.1 & 30.6 \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{Impact of language similarity on cross-lingual transfer.} We simulate a low-resource language scenario by using only 5 hours of Italian CommonVoice data and add 50 hours from another language for pretraining. We fine-tune on 1 hour of Italian supervised data. \label{tab:lang_sim}}
       \vspace{-0.4cm}
        \end{center}
    \end{table*}
}

% Low-resource language and language similarity
\newcommand{\insertmls}{
    \begin{table*}[b]
        \begin{center}
            % \scriptsize
            \resizebox{0.8\linewidth}{!}{
            \begin{tabular}[h!]{l|cl|cccccccc}
            \toprule
                Model & {\bf \#pt} & {\bf \#ft} & {\bf en }& {\bf de }& {\bf nl }& {\bf fr }& {\bf es }& {\bf it }& {\bf pt} & {\bf pl} \\
                \midrule
                \midrule
                \multicolumn{3}{l|}{Number of training hours} & 44.7k & 2k & 1.6k & 1.1k & 918 & 247 & 161 & 104  \\
                \midrule
                \midrule
                LibriVox & 1 & 1-1h & 13.2 & 25.5 & 30.3 & 37.0 & 22.5 & 23.3 & 37.8 & 38.4 \\
                LibriVox & 1 & 1-10h & 10.6 & 14.5 & 19.6 & 19.6 & 13.5 & 16.7 & 25.0 & 32.0 \\
                \midrule
                XLSR-53 & 53 & 1-1h & 17.3 & 10.6 & 15.6 & 17.0 & 10.4 & 15.1 & 21.4 & 31.9  \\
                XLSR-53 & 53 & 1-10h & 14.6 & 8.4 & 12.8 & 12.5 & 8.9 & 13.4 & 18.2 & 21.2   \\
                XLSR-53 & 53 & 1-100h & 13.2 & 7.4 & 10.9 & 9.8 & 7.9 & 12.0 & 15.7 &  18.9  \\
                XLSR-53 & 53 & 1-full & - & 7.0 & \bf 10.8 & 7.6 & 6.3 & \bf 10.4 & \bf 14.7 & \bf 17.2 \\
                \midrule
                \cite{pratap2020mls} &  - & 1-full & \bf 5.88 & \bf 6.49 & 12.02 & \bf 5.58 & \bf 6.07 & 10.54 & 19.49 & 20.39 \\

                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{Word error rate (WER) results on MLS.} We fine-tune XLSR-53 on 1h, 10h, 100h and full data to evaluate the few-shot capability of the model on the MLS languages, and compare it to the baseline from \cite{pratap2020mls} which leverages the full supervised data (i.e. 44.7k hours on English), as well as the LibriVox model from \cite{baevski2020wav2vec2}. We use a 4-gram KenLM model. \label{tab:mls}}
       \vspace{-0.4cm}
        \end{center}
    \end{table*}
}

% Description of CommonVoice data
\newcommand{\insertCVdata}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{0.8\linewidth}{!}{
            \begin{tabular}[b]{l|cccccccccc|c}
            \toprule
            \bf CommonVoice & {\bf es} & {\bf fr} & {\bf it} & {\bf ky} & {\bf nl} & {\bf ru} & {\bf sv} & {\bf tr} & {\bf tt} & {\bf zh} & {\bf $\sum$}\\
                \midrule
                Pretraining data & 168h & 353h & 90h & 17h & 29h & 55h & 3h & 11h & 17h & 50h & 793h \\
                Training data& 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 10h \\
                Valid data & 20m & 20m & 20m & 20m & 20m & 20m & 20m & 20m & 20m & 20m & 3h \\
                Test data & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 1h & 10h \\
                Vocabulary size & 39 & 38 & 60 & 39 & 53 & 50 & 41 & 47 & 44 & 63 & 474 \\
                \bottomrule
            \end{tabular}
            }
            \caption{\textbf{CommonVoice data statistics}: amount of unsupervised, supervised data, and vocab size.
            \label{tab:cv_data}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}


% Description of BABEL data
\newcommand{\insertBABELdata}{
    \begin{table*}[h!]
        \begin{center}
            % \scriptsize
            \resizebox{1\linewidth}{!}{
            \begin{tabular}[b]{l|lccccccccccccc|c}
            \toprule
              \bf BABEL & {\bf bn} & {\bf zh} & {\bf ka} & {\bf ht} & {\bf ku} & {\bf ps} & {\bf ta} & {\bf tr} & {\bf tp} & {\bf vi} & {\bf as} & {\bf tl} & {\bf sw} & {\bf lo} & {\bf $\sum$}\\
                \midrule
                Pretraining data & 56h & 130h & 46h & 61h & 38h & 71h & 63h & 70h & 36h & 79h & 55h & 76h & 30h & 59h & 870h \\
                Training data & 56h & 130h & 46h & 61h & 38h & 71h & 63h & 70h & 36h & 79h & 55h & 76h & 30h &  59h & 870h \\
                Valid data & 6h & 15h & 5h & 7h & 4h & 8h & 9h & 8h & 4h & 9h & 6h & 7h & 4h & 7h & 98h \\
                Test data & 10h & 18h & 12h & 11h & 10h & 10h & 11h & 10h & 10h & 11h & 10h & 12h & 11h & 11h & 155h\\
                Vocabulary size & 69 & 3437 & 37 & 63 & 67 & 53 & 52 & 69 & 58 & 135 & 69 & 52 & 59 & 57 & 4277 \\
            \bottomrule
            \end{tabular}
            }
            \caption{\textbf{BABEL data statistics}: amount of unsupervised, supervised data, and vocab size.
            \label{tab:bbl_data}}
        \end{center}
       \vspace{-0.4cm}
    \end{table*}
}

% Analysis plots (shared vocabulary)
\newcommand{\insertXLSR}{
\begin{table*}[h!]
\begin{minipage}[t]{0.48\linewidth}
	\begin{center}
          %\includegraphics[width=\linewidth]{content/xlmroberta_transfer_dilution.pdf}
          \includegraphics[width=1\linewidth]{figure/model.pdf}
        \captionof{figure}{\textbf{\wvpp} We use the \wvpp{} architecture introduced by \citet{baevski2020wav2vec2} as a bottleneck architecture to encode multiple languages at once. The quantizer of the speech input is trained jointly with a masked language model Transformer during pretraining. \label{fig:modelone}}
        \vspace{-0.2cm}
	\end{center}
\end{minipage}
\hfill
\begin{minipage}[t]{0.48\linewidth}
	\begin{center}
          %\includegraphics[width=\linewidth]{content/xlmroberta_transfer_dilution.pdf}
          \includegraphics[width=0.85\linewidth]{figure/xlsr.pdf}
        \captionof{figure}{At inference time, our model encodes raw wave forms coming from multiple languages into a shared multilingual token embedding space. The speech "word embeddings" are then forwarded to a Transformer architecture. Close languages share more discrete tokens. \label{fig:modeltwo}}
        \vspace{-0.2cm}
	\end{center}
\end{minipage}
%\vspace{-0.3cm}
\end{table*}
}

% Analysis plots (shared vocabulary)
\newcommand{\insertXLSRtwo}{
\begin{table*}[t]
	\begin{center}
          %\includegraphics[width=\linewidth]{content/xlmroberta_transfer_dilution.pdf}
          \includegraphics[width=\linewidth]{figure/xlsr.pdf}
        \captionof{figure}{\textbf{The \xlsr{} approach.} A shared quantization module over feature encoder representations produces multilingual quantized speech units whose embeddings are then used as targets for a Transformer trained by contrastive learning. The model learns to share discrete tokens across languages, creating bridges across languages. Our approach is inspired by \citet{devlin2018bert,lample2019xlm} and builds on top of \wvpp~\citep{baevski2020wav2vec2}. It requires only raw unlabeled speech audio in multiple languages.
        % \xlsr{}} learns unsupervised cross-lingual speech representations using a constrastive loss for masked time-steps over quantized latent speech representations.
        % We pretrain a single model on batches of speech audio in multiple languages. 
        % The latent representations 
        % \textbf{\xlsr{}} learns unsupervised cross-lingual speech representations using \wvpp{}~\cite{baevski2020wav2vec2} as a bottleneck architecture (left figure). We train a quantizer of the speech input jointly with a masked language model Transformer. During pretraining, we sample batches of speech audio from multiple languages, and share all parameters. The quantizer builds multilingual quantized latent speech representations (right figure), which the model learns to share across languages depending on language similarity. The XLSR approach can leverage speech audio from multiple languages to build better representations, in particular for low-resource languages. 
        \label{fig:modelone}}
        \vspace{-0.2cm}
	\end{center}
\end{table*}
}


% Analysis plots (shared vocabulary)
\newcommand{\insertAnalysistwo}{
\begin{table*}[b]
	\begin{minipage}[t]{0.3\linewidth}
	\begin{center}
          \includegraphics[width=1.1\linewidth]{figure/cv1_analysis.pdf}
        \captionof{subfigure}{CV-12 model.\label{fig:analysis_cv1}}
        \vspace{-0.2cm}
	\end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.3\linewidth}
	\begin{center}
          \includegraphics[width=1.1\linewidth]{figure/cv2_analysis.pdf}
        \captionof{subfigure}{CV-12 model + zh-HK.\label{fig:analysis_cv2}}
	\end{center}
    \end{minipage}
    \hfill
	\begin{minipage}[t]{0.3\linewidth}
	\begin{center}
          \includegraphics[width=1.1\linewidth]{figure/bbl_analysis.pdf}
        \captionof{subfigure}{BABEL-17 model.\label{fig:analysis_bbl}}
	\end{center}
    \end{minipage}
\captionof{figure}{\textbf{Visualization of language similarities learned by the model}  Figure (a) shows that our CommonVoice model trained on 12 languages (CV-12) can choose to cluster languages in the shared token embedding space. By adding Chinese-HongKong (zh-HK), we show in Figure (b) that a language can share fewer tokens with other languages and thus be isolated. Figure (c) shows for 17 languages of BABEL that clusters can correspond to similar language like Bengali and Assamese. \label{fig:analysis}}
\end{table*}
}

% Analysis plots (shared vocabulary)
\newcommand{\insertAnalysis}{
\begin{figure}[ht]
\begin{subfigure}{.32\textwidth}
  \centering
  % include first image
    \includegraphics[width=1\linewidth]{figure/cv1_analysis.pdf}
  \caption{CV-12 model.}
  \label{fig:analysis_cv1}
\end{subfigure}
\hfill
\begin{subfigure}{.32\textwidth}
  \centering
  % include second image
    \includegraphics[width=1\linewidth]{figure/cv2_analysis.pdf}
  \caption{CV-12 model + zh-HK.}
  \label{fig:analysis_cv2}
\end{subfigure}
\hfill
\begin{subfigure}{.32\textwidth}
  \centering
  % include second image
    \includegraphics[width=1\linewidth]{figure/bbl_analysis.pdf}
  \caption{BABEL-17 model.}
  \label{fig:analysis_bbl}
\end{subfigure}
\caption{\textbf{Visualization of language similarities learned by the model}  Figure (a) visualizes the shared discrete latent speech representations across languages for a model trained on 12 CommonVoice languages (CV-12). Figure (b) shows that adding Chinese-HongKong (zh-HK) shares relatively few latents with other languages. Figure (c) is for a model trained on 17 BABEL languages and illustrates that clusters can correspond to similar languages like Bengali and Assamese.}
\label{fig:analysis}
\end{figure}
}

